Isolario: a Do-ut-des Approach to Improve the Appeal of BGP Route Collecting

The incompleteness of data collected from BGP route collecting projects is a well-known issue which potentially affects every research activity carried out on the analysis of the Internet inter-domain routing. Recent works explained that one of the possible solutions is to increase the number of ASes feeding these projects from the Internet periphery, in order to reveal the hidden portion of peering connectivity of their upstream providers. The main problem is that these projects are currently not appealing enough for the network administrators of these ASes, which are typically not aware of their existence or not interested enough to share their data. Our contribution is Isolario, a project based on the do-ut-des principle which aims at persuading network administrators to share their routing information by offering services in return, ranging from real-time analyses of the incoming BGP session(s) to historic analyses of routing reachability. To the best of our knowledge, Isolario is the only route collecting project publicly available which offers a set of services to its users to encourage their participation, aiming at increasing the amount of BGP data publicly available for research purposes.

==> isolario.tex <==
\section{Isolario}
\label{sec:arch}

As described in~\cite{Gregori12}, most of the ASes participating in any BGP 
route collecting project with a full routing table are large organisations, 
often worldwide ISPs, which exploit route collectors to advertise the quality of
their inter-domain routing free of charge. Despite their importance, these kinds
of organisations are just a small percentage in the Internet ecosystem, which is
mostly populated by smaller companies, like regional ISPs or local CDNs. Given 
the economic relationships ruling the Internet~\cite{Gao01} though, these latter
companies are also the most important sources of information to reveal 
characteristics of the Internet previously unknown via their hypothetical BGP 
feed to a route collector~\cite{Gregori12}. For example, most of these ASes 
would be able to discover part of the peering connections established at IXPs by
them directly (or by their providers), thus potentially contributing to turn 
upside-down the hierarchical view of the Internet~\footnote{According to the 
one-shot study done in~\cite{Ager12}, it is possible to find more than 50K 
active BGP connections hidden at the sight of Route Views and RIS on a single 
European IXP.}. 

%Isolario's main challenge is to attract into route collecting smaller ISPs and 
%CDNs -- which do not share the same resources of their worldwide counterparts -- 
%by focusing mostly on finding services that can be useful for their network administrators.
Isolario offers to network administrators a dedicated infrastructure to provide them both 
\textit{real-time} and \textit{historic} services focused on their inter-domain 
routing, in exchange for (at least) one BGP session from one of the ASBRs managed by the network administrators. The incoming BGP flow(s) will be used by Isolario
as input to the network administrator dedicated services and, at the same time, 
will be stored in MRT format and made available on a public online repository. 
In this section we will describe the Isolario architecture and we will focus on 
the techniques applied to provide to Isolario users responsive and efficient 
services.


\input{architecture}

\input{need_for_speed}

